A Hypergradient Approach to Robust Regression without Correspondence

We consider a variant of regression problem, where the correspondence between input and output data is not available. Such shuffled data is commonly observed in many real world problems. Taking flow cytometry as an example, the measuring instruments may not be able to maintain the correspondence between the samples and the measurements. Due to the combinatorial nature of the problem, most existing methods are only applicable when the sample size is small, and limited to linear regression models. To overcome such bottlenecks, we propose a new computational framework -- ROBOT -- for the shuffled regression problem, which is applicable to large data and complex nonlinear models. Specifically, we reformulate the regression without correspondence as a continuous optimization problem. Then by exploiting the interaction between the regression model and the data correspondence, we develop a hypergradient approach based on differentiable programming techniques. Such a hypergradient approach essentially views the data correspondence as an operator of the regression, and therefore allows us to find a better descent direction for the model parameter by differentiating through the data correspondence. ROBOT can be further extended to the inexact correspondence setting, where there may not be an exact alignment between the input and output data. Thorough numerical experiments show that ROBOT achieves better performance than existing methods in both linear and nonlinear regression tasks, including real-world applications such as flow cytometry and multi-object tracking.

==> tex_files/broader.tex <==
%!TEX root = ./iclr2021_conference.tex

\section{Broader Impact}

% RWOC has many real-world applications. Specifically, we divide the applications into two cases: when the measuring instruments are unable to preserve the correspondence between the samples and measurements, and when the data are obtained from multiple sources. In the former case, besides the physical experiments we mentioned in the introduction, the proposed method is also applicable to many vision-based tasks. Examples includes pose/correspondence estimation and multi-object tracking, which plays a central role in robotics and autonomous driving. 

This paper makes a significant contribution to extending the frontier of regression problems without full supervision, by developing a new algorithm with better scalability and efficiency for the RWOC problem, and hence increase computational feasibility.
To the best of our knowledge, our method is one of the first few principled approaches to consider the robust RWOC where the input and the output are not exactly aligned. 
Moreover, our results are also the first to explicitly exploit the interaction between the correspondence and the regression model in RWOC problems. This is in sharp contrast with current practices, which mostly optimize the correspondence and the regression model alternatingly.

We remark that ROBOT has wide applications in autonomous driving, robotics, and privacy protection in social science. Especially for social science, there has been a notably increasing need to protect user privacy in databases. The proposed approach is capable of learning a good model from multiple databases without knowing the identity of the users. This lowers the need for privacy information when collecting data, which in turn helps protect the privacy of the users.

